Certain and Approximately Certain Models for Statistical Learning

Real-world data is often incomplete and contains missing values. To train accurate models over real-world datasets, users need to spend a substantial amount of time and resources imputing and finding proper values for missing data items. In this paper, we demonstrate that it is possible to learn accurate models directly from data with missing values for certain training data and target models. We propose a unified approach for checking the necessity of data imputation to learn accurate models across various widely-used machine learning paradigms. We build efficient algorithms with theoretical guarantees to check this necessity and return accurate models in cases where imputation is unnecessary. Our extensive experiments indicate that our proposed algorithms significantly reduce the amount of time and effort needed for data imputation without imposing considerable computational overhead.

==> Supplementary_Materials.tex <==
\section{Supplementary Materials}
\subsection{Proof to Algorithm \ref{alg:ACM-linear_regression}}
Algorithm \ref{alg:ACM-linear_regression} can be splitted to three steps below.

\noindent
{\textbf{Step 1: Finding interval-formatted orthogonal basis} Based on the Gram-Schmidt process \cite{leon2013gram}, we find the first basis vector $\mathbf{b}_1 = \mathbf{z}_1$, and then the second basis vector $\mathbf{b}_2 = \mathbf{z}_2 - \text{proj}_{\mathbf{b_1}}(\mathbf{z_2})$, so on so forth till $\mathbf{b}_{d}$. The last basis vector $\mathbf{b}_d = \mathbf{z}_d - \text{proj}_{\mathbf{b_1}}(\mathbf{z_d}) - ... - \text{proj}_{\mathbf{b_{d-1}}}(\mathbf{z_d})$. Projecting one interval vector onto another interval vector is efficiently implemented through an existing interval arithmetic solution \cite{jaulin2001interval}. As a result, we find orthogonal basis ($\mathbf{b}_1, ..., \mathbf{b}_d$) where $\mathbf{b}_i = [b_{i1}, ..., b_{in}]^T$ is uncertain but bounded by
\[
b_{i1}^{min} \leq b_{i1} \leq b_{i1}^{max}, ..., b_{in}^{min} \leq b_{in} \leq b_{in}^{max}
\]


\noindent
{\textbf{Step 2: Projecting Label Vector onto Orthogonal Basis} 
We perform linear regression with orthogonal basis vectors, and get linear coefficients $\beta_1, ..., \beta_d$. Due to the orthogonality, linear regression is simply computing inner products between the label vector and each basis vector:
\[
\mathbf{\beta}^T = [\beta_1, \ldots, \beta_d] = \mathbf{y}^\intercal \cdot [\mathbf{b}_1, \ldots, \mathbf{b}_d]
\]
Here, $\beta_1, \ldots, \beta_{d}$ are interval values because basis vectors are interval vectors. Again, the inner product operations above can be efficiently implemented through the existing solution. Denote $\beta_d = [\beta_d^{min}, \beta_d^{max}]$ where $\beta_d^{min} \leq \beta_d \leq \beta_d^{max}$. So far, we have passed uncertainty from missing data to linear regression model by $\mathbf{\beta}$. However, the linear regression model $\mathbf{\beta}$ is with respect to the orthogonal basis instead of the original training data. Hence, we need to transform $\mathbf{\beta}$ to $\mathbf{w}$, which is the linear regression model with respect to the original training data $\mathbf{X}$. 

\noindent
{\textbf{Step 3: Determining the bounds for linear regression models} From Step 2, we get the optimal linear regression model $\mathbf{\beta}$ such that:

\[
\mathbf{y} = \beta_1 \cdot \mathbf{b}_1 + ... + \beta_d \cdot \mathbf{b}_d + \mathbf{r}
\]

where $\mathbf{r}$ is the minimal regression residue. Now, we replace $\mathbf{b}_1, ..., \mathbf{b}_d$ with $\mathbf{z}_1, ..., \mathbf{z}_d$ to get optimal model $\mathbf{w}$ with respect to $\mathbf{X}$:

\[
\mathbf{y} = w_1 \cdot \mathbf{z}_1 + \dots + w_d \cdot \mathbf{z}_d + \mathbf{r}
\]

In this step, we find the model parameters in the format of intervals. As a result, we get bounds for each model parameter: $w_1^{min} \leq w_1 \leq w_1^{max}, ..., w_d^{min} \leq w_d \leq w_d^{max}$. Finally, the Euclidean distance between two possible models is bounded by $e = \sqrt{\sum_{i=1}^{d} (w_i^\text{max} - w_i^\text{min})^2}$.

% \subsection{Refresher for Support Vector Machines}
% \paragraph{}
% Support Vector Machine (SVM) was first introduced by Vapnik et al in 1992. SVMs are a set of supervised machine learning methods used for solving classification and regression problems. The premise of SVMs is that it uses a hypothesis space of a linear function in a higher dimensional feature space to make it’s predictions. By using kernels, all necessary computations can be performed in the input space thus avoiding expensive high dimensional computations. SVM gained popularity in the community for being highly explainable and effective in solving complex tasks with comparable accuracy to complex neural networks. 

% The goal of SVM is to find the best line or decision boundary that can be used to separate the space into classes. For higher dimensions the line is replaced by a hyperplane. SVM uses the points from the different classes which have the least distance between them, these points are termed as support vectors. Let’s consider the Figure 6 below, we want to define a model which can correctly classify people who are at a risk of being overweight based on their height and weight. The two support vectors are utilized to maximize the margin and form the decision boundary. This example uses the Linear Kernel which is defined by the formula.\\

% f(X) = $w^T$ * X + b\\

% In this equation, w is the weight vector that you want to minimize, X is the data that you're trying to classify, and b is the linear coefficient estimated from the training data. This equation defines the decision boundary that the SVM returns.

% \begin{figure}[H]
%   \centering
%     \includegraphics[scale=0.65]{images/SVM.png}
%     \caption{Linear hard margin Support Vector Machine}
%   \hfill
% \end{figure}








==> section0_response_to_reviewer_comments.tex <==
\pagestyle{empty}

\setcounter{page}{1}
\begingroup
  \centering
  \Large {\bf Responses to Reviewers' Comments}\\[0.0em]
\endgroup

We thank the reviewers for their insightful comments, based on which we have made significant changes to improve the paper. 
The titles of new sections and paragraphs in the paper are highlighted in {\color{red} red}. 

To address the reviewers' comments, we have added a new section about approximately certain models, Section 8, and reported our empirical studies on eight (8) new real-world datasets on both certain and approximately certain models in the revised submission. Given these additional materials and due to the lack of space, we have removed all proofs from the revised manuscript. 
For the same reason, we have also removed our empirical studies on purely synthetic data from the revised submission.
If the submission gets accepted, we will include these in a technical report and provide its link in the paper. 


\section*{Responses to the Meta-reviewer’s Comments (MR)}

\begin{itemize}
    \item[\textbf{[MR 1]}]  {\it Practical motivation for the specific problem formulation studied in the paper.}\\
    
    \noindent\textbf{[Response]} Please refer to our responses to comments O1 and O4 of Reviewer \#1 and comments O1.a and O1.b of Reviewer \#2.\\
    
    %When a dataset has missing values, there are many different imputations to repair the dataset. Training models with all possible repairs individually and then analyzing the models is usually not practical. In our paper, we check if there is a model that is accurate or sufficiently accurate for all repairs. If yes, users can save a huge amount of energy for data imputation because it is unnecessary. We formulate certain models that are optimal (i.e., having minimal training loss) for all repairs. Relaxing certain models, we formulate approximately certain models that are sufficiently close to optimal (i.e., having training loss sufficiently close to the minimum). Details can be found in Sections 3 and 8.\\

    \item[\textbf{[MR 2]}] {\it Comparison with more up-to-date and sophisticated imputation techniques than ActiveClean. }\\
    
    \noindent\textbf{[Response]} We have compared our method to three additional imputation techniques some of which are more recent and sophisticated than ActiveClean: 1) {\it mean imputation} that is used often in practice, 2) {\it KNN imputation} \cite{articleKNN,pmlr-v97-mattei19a}, and 3) {\it deep-learning based imputation, MIWIE} \cite{pmlr-v97-mattei19a}. Additionally, we have also included the results of the simple technique of ignoring missing values (NI). These methods are explained in Section~\ref{sec:algorithms_for_comparison}. \\
    
    \item[\textbf{[MR 3]}] {\it Questions about the utility of and qualify (i.e., approximation guarantee) of approximation. Lack of experimental evidence to demonstrate the quality.}\\
    
    \noindent\textbf{[Response]} Please refer to our response to comment O3 of Reviewer \#1.\\
    %We add a section (Section 8) to define approximately certain models, and discuss algorithms to check and learn the models. Experimental results about approximately certain models on real-world incomplete data are also presented and discussed in Section 9.\\
    
    \item[\textbf{[MR 4]}] {\it Relaxing certain model to invariance of test predictions (for classification tasks).}\\
    
    \noindent\textbf{[Response]} Please refer to our response to comment O4 of Reviewer \#1.\\
    
    \item[\textbf{[MR 5]}] {\it Generality of value missing mechanisms studied.}\\
    
    \noindent\textbf{[Response]} Please refer to our responses to comments O1 and O4 of Reviewer \#1, comment MR8 of the meta-review, and comment O1 of Reviewer \#3.\\ 

    %Our approach applies to all missing mechanisms since the formulations and algorithms in the paper do not assume any specific missing mechanism. In Section 9, we study certain and approximately certain models over real-world datasets with a variety of missing mechanisms, demonstrating the coverage of our approach. Table 2 provides a summary of these datasets.\\
    
    \item[\textbf{[MR 6]}] {\it What fraction of datasets admit a certain model? }\\
    
    \noindent\textbf{[Response]} In Section 9 of the revised submission, we have added an extensive empirical study using eight real-world datasets with missing values to answer this question for both certain and approximately certain models. Our studies indicate that certain and approximately certain models appear quite frequently in real-world datasets. Please refer to Sections \ref{sec:results-original-corruption} and \ref{sec:results-random-corruption} for detailed analysis.\\  
    %Two of them admit certain models, and of course, also admit approximately certain models. For the rest of the six datasets, two admit approximately certain models.
    
    \item[\textbf{[MR 7]}] {\it Comparison with natural logical baselines identified by reviewers.}\\
    
    \noindent\textbf{[Response]} Please refer to our response to comment MR2 in the meta-review.\\
    
    \item[\textbf{[MR 8]}] {\it Need to improve experiments and make them more comprehensive to cover unanswered questions.}\\
    
    \noindent\textbf{[Response]} We have added empirical studies of eight real-world datasets that originally contain missing values with different degrees of missingness in Section 9 of the revised submission. We have also empirically evaluated four new competing techniques and reported their results in the same section.   
    
    
\end{itemize}

\section*{Responses to the Comments of Reviewer \#1}
\begin{itemize}
    \item[\textbf{[O1]}]  \textit{My biggest concern with this work is that it does not give any answer to the following question: how often do certain models exist in practice? This is really important, because on first look, the definition of a certain model seems very restrictive. In particular, the definition asks for the optimal model to remain "exactly" the same, independent of the imputation of the missing values. This may be stronger than we want for practical purposes, because even if the model is slightly different, that may be sufficient for our purposes. But if such certain models exist in real-world datasets and tasks, then the notion would be useful}\\
    
    \textbf{[Response]} We have followed the reviewer’s suggestion and added an extensive empirical study using eight new real-world datasets that originally contain missing values to Section 9 whose goal is to find out the frequency of certain models in real-world datasets. Our results indicate that certain models appear in quite a few datasets in practice. Section \ref{sec:results-original-corruption} provides details of this analysis.
    Moreover, we have introduced a relaxed notion of certain models called approximately certain models, in Section \ref{sec:Approximate}. 
    We report an empirical study on the existence of these models in real-world data in Section \ref{sec:results-original-corruption}  of the revised submission.\\
     
    \item[\textbf{[O2]}] \textit{ I don't find the comparison with ActiveClean very meaningful. Reporting the cleaning costs does not tell us anything about the proposed approach, which has 0 cleaning cost. The runtime results are somewhat more interesting.}\\
    
     \textbf{[Response]} Our objective is to eliminate data cleaning efforts without impacting the training accuracy when possible. Hence, we compare our method with the state-of-the-art technique that also aims at reducing the amount of data cleaning effort. To the best of our knowledge, ActiveClean is the most well-known method in this area that supports the same models as ours. In comparison, ActiveClean cleans many training examples, which require a great deal of manual effort to find and deploy the proper imputation methods. This indicates that as opposed to our method, ActiveClean cannot find the minimum number of required cleaning operations in these cases. \\
     % In Table 2, we report 0 cleaning costs from our method because certain models exist.
    
    \item[\textbf{[O3]}] \textit{Section 7 seems out of place for two reasons. First, it does not really compute a certain model, but approximates it. But if it makes sense to approximate it, then why not do it in general? And what guarantee do we achieve? Second, there are no experimental results for this case (which also seems to be the one of most practical interest).}\\
    
     \textbf{[Response]} Our goal is to compute the certain model exactly if possible. Due to the non-convexity and complexity of DNNs, it is difficult to compute their certain models precisely. Hence, we use techniques that approximate DNNs using simpler models (Kernel SVMs) accurately and approximate certain models for DNNs by computing them for these proxies. 
     Since we can compute certain models precisely for other models, there is no reason to approximate them for these models.
     We have followed the reviewer's comments regarding experimental results and reported empirical studies of the methods proposed in Section \ref{sec:DNN} in Section \ref{sec:experimental-evaluation} of the revised submission.\\
    
    \item[\textbf{[O4]}] \textit{ For classification tasks, it would make sense to compare with the approach of checking whether the test point predictions remain the same (instead of the optimal model). This is a more relaxed notion of certainty, but it would lead to even less need for cleaning.}\\

    \textbf{[Response]} We have proposed a new relaxed version of certain models called approximately certain models in Section \ref{sec:Approximate} of the revised version that reflects this idea. The expected loss of an approximately certain model is close to the minimal loss for all repairs of the training data. The standard assumption for the statistical models discussed in our work is that the training and testing data are samples from the same distribution. Thus, the expected loss of a model, i.e., its prediction quality, on training data must be equal to or accurately approximate its expected loss on testing data. \\

    \item[\textbf{[D\&I]}] \textit{All the figures use color as the only distinguishing characteristic; this can be easily fixed.}\\
    
    \textbf{[Response]} Compliance has been addressed for all figures in the revised submission.\\
    
    \item[\textbf{[M1]}] \textit{The algorithm boxes do not give much additional information compared to the theorems describing the conditions; I would suggest removing them (or some of them).}

    \textbf{[Response]} Many algorithm boxes offer concise implementation details beyond the mathematical formulations in the theorems. Following the suggestion, we have removed Algorithm 4 for SVM with RBF kernel because its general idea is very similar to Algorithm 3 for SVM with polynomial kernel. \\
    
    \item[\textbf{[M2]}] \textit{Some relevant literature is missing from the paper:}
    
    \begin{enumerate}
        \item "Certifiable Robustness for Nearest Neighbor Classifiers", Austen Z. Fan, Paraschos Koutris, ICDT 2022.
        \item "Proving Data-Poisoning Robustness in Decision Trees", Samuel Drews, Aws Albarghouthi, Loris D'Antoni, PLDI 2020.\\
    \end{enumerate}
     \textbf{[Response]} We have added and discussed these references in Sections \ref{sec1} and \ref{sec2} of the revised submission, respectively.
    
    %\item[\textbf{[M3]}] \textit{What other models can be handled with the proposed technique? What are the limitations?}
    %\\
    % \textbf{[Response]}
\end{itemize}

\section*{Responses to the Comments of Reviewer \#2}
\begin{itemize}
    \item[\textbf{[O1.a]}]  \textit{The real world datasets do not have missing values and missing values are injected uniform at random which is not realistic. There are plenty of open datasets with missing values that could be used instead. It is not clear whether results for missing at random translate to other types of missingness mechanisms. While determining what mechanism did generate the missing values is hard, this is not required when real world datasets with missing values are used.}\\
    
    \textbf{[Response]} Please refer to our response to MR 8.\\
    
    \item[\textbf{[O1.b]}]  \textit{An interesting metric that is not evaluated is what is the fraction of datasets for which certain models exist (if that fraction is low, then the approach is not very useful). Furthermore, it would be interesting to compare against simpler imputation techniques in terms of runtime and accuracy.}\\
    
    \textbf{[Response]} Please refer to our responses to comment O1 of Reviewer \#1 and comment MR2 in the meta-review. \\ 
 
    
    \item[\textbf{[O1.c]}]  \textit{As computing certain models often boils down to using the standard learning algorithm over a reduced training dataset that does not include incomplete instances and features, it would be interesting to measure the accuracy of this approach against standard imputation techniques when no certain model exists (is the check for certainty necessary in the end)}\\
    
\textbf{[Response]} Please refer to our response to comment MR2 in the meta-review.\\
    
    \item[\textbf{[O2]}] \textit{The aspect that certain models basically correspond to strategies that are already widely used (like dropping incomplete features / instance) should be highlighted more. Also I am wondering whether some of the results the authors derived are already known in the ML community?}\\
    
    \textbf{[Response]} We have followed the reviewer's comment and clarified this connection in Section \ref{sec:certain-models} of the revised submission. To the best of our knowledge, these results are not known in the ML community.

\end{itemize}


\section*{Responses to the Comments of Reviewer \#3}
\begin{itemize}
    \item[\textbf{[O1]}]  \textit{My primary concern regarding this work is its motivation. Specifically, while the paper proposes a method for identifying certain models that can be beneficial when they exist, a critical question is: how probable is it for real-world scenarios to have these specific models and the capacity to avoid imputation? Additionally, several related questions to be answered. Firstly, how does the class of models impact the likelihood of enjoying certain models, such as whether more expressive models are less likely to exhibit them? Secondly, what characteristics of the data influence the probability of encountering these models, such as the number of attributes, the number of samples, or the domain sizes?}\\
    
    \textbf{[Response]} Firstly, we have included an extensive empirical study using eight new real-world datasets in Section \ref{sec:experimental-evaluation} of the revised submission that answers these questions. Please refer to our responses to comment O1 of Reviewer \#1 for more information about these studies. Secondly, we have found three major characteristics for datasets that affect the chance of admitting certain and approximately certain models. 1) Observed in experiments of randomly corrupted datasets with different missing factors in Section \ref{sec:results-random-corruption}, the likelihood of certain and approximately certain models existing increases as the missing factor decreases. 2) In our experiments of real-world datasets with inherent missingness in Section \ref{sec:results-original-corruption}, we have observed that certain and approximately certain models are more likely to exist in regression tasks when the number of features is large, and in classification tasks when the number of examples is large. 3) A dataset has a higher chance to admit certain and approximately certain models when its incomplete features are not relevant to the label based on common sense, such as the COVID dataset in our experiment.\\
    
    
    \item[\textbf{[O2]}]  \textit{Linked to the concerns raised in O1, the experimental analysis lacks a well-designed experiment that can address the question in O1 effectively. While the authors argue and demonstrate that checking for certain models incurs minimal overhead, justifying its worth, it remains crucial to demonstrate how often this checking leads to improved performance in real-world data scenarios. The datasets presented in the experimental section predominantly consist of synthetic data (both data and missing values are generated) or data with missing values are injected. Consequently, a lingering question still is: what is the likelihood of encountering certain models in real-world applications?}\\
    
    \textbf{[Response]} Please refer to our responses to comment O1 of Reviewer \#1. \\
    
    \item[\textbf{[O3]}] \textit{Multiple state-of-the-art imputation methods should be employed to compare the training and imputation costs. Active Clean is a relatively dated technique in this context.}\\
    
    \textbf{[Response]} Please refer to our response to comment MR2 in the meta-review.

\end{itemize}

==> section10_Lessons_learned.tex <==
\section{Lessons Learned}\label{sec9}
The algorithms for linear regression and SVM are designed to determine if missing features or training examples are irrelevant or redundant when minimizing training loss, given non-missing data. In practice, data irrelevance and redundancy are often addressed after handling missing data because missing data is typically assumed to be significant. In the paper, our algorithms are focused on cases where missing features/training examples are irrelevant or redundant irrespective of the missing data's actual values. 

When dealing with certain models in practical ML problems, three key issues can arise. Firstly, while certain models may allow for the omission of missing features or training examples, this approach can lead to overfitting, particularly in datasets with a high number of missing values. Secondly, checking certain models may not be feasible in practice due to the strict optimality requirements of all repairs. Thirdly, certain model algorithms rely on constraints in the hypothesis space, such as linearity in linear regression, making it difficult to efficiently verify certain models for flexible ML models like neural networks.

To overcome these challenges, it is crucial to develop a relaxed optimality condition and leverage non-missing values in missing features/training examples. Additionally, probabilistic models with repair sampling can facilitate the development of efficient algorithms for general ML models. Finally, given the importance of data cleaning in many scenarios, combining certain model algorithms with popular progressive data cleaning frameworks may prove effective in real-world datasets.



==> section3_background_version1.tex <==

\section{Background}\label{sec3}
%This paper presents examples of supervised learning including linear regression and SVM. The ideas can also be applied to unsupervised learning models as the general idea shares.
\begin{table}[h]
  \caption{A training dataset for rain prediction}
  \label{tab:missing_value}
  \begin{tabular}{cccl}
    \toprule
    & Temperature  & Humidity & Rain (1) or No Rain (-1)\\
    \midrule
    Seattle & 65 & 80 & 1\\
    New York  & 50 & $null$ & -1\\
    \bottomrule
  \end{tabular}
  % \label{table:1}
\end{table}
\subsection{Supervised Learning}

\paragraph{{\bf Training Examples}} Consider a relation with $n$ tuples. {\it For instance, the relation in \autoref{tab:missing_value} has two tuples(rows)}. For a machine learning problem, the $n$ tuples are considered training examples. {\it \autoref{tab:missing_value} has 2 training examples (Seattle, New York)}. We denote a single training example as \textbf{x} and a collection of $n$ training examples as a vector $[\textbf{x}_{1}, ...,\textbf{x}_{n}]$.

\paragraph{{\bf Label}}The column(attribute) of a dataset(relation) we are using an ML algorithm to make predictions on is called a label. {\it For instance, Rain or No Rain column in \autoref{tab:missing_value}}. We denote a label as $y$ and the entire label column with $n$ labels as a vector $\textbf{y} = [y_{1}, ..., y_{n}]$.

\paragraph{{\bf Features}} The remaining $d$ columns of a dataset are called features. {\it For instance, Temperature and Humidity are the two features in \autoref{tab:missing_value}}. We denote a single feature as \textbf{z} and $d$ features as a vector $[\textbf{z}_{1}, ..., \textbf{z}_{d}]$.To simplify our exposition, we assume all feature values come from a set of real numbers $\mathbb{R}$.


\paragraph{{\bf Training Set}} The dataset (e.g., \autoref{tab:missing_value}) as a whole is called a training set. Formally, given $n$ training examples, a training set consists of an input matrix $\textbf{X} =[\textbf{x}_{1}, ..., \textbf{x}_{n}]$ and a label vector $\textbf{y} = [y_{1}, ..., y_{n}]$.  Since a training example is made up of $d$ features, a training example in terms of the input matrix is essentially a vector $\textbf{x}_i = [x_{i1}, ..., x_{id}]$. Here $x_{ij}$ denotes the $j^{th}$ feature in the $i^{th}$ example of the matrix. 


\paragraph{{\bf Target Function}} For a vector of $n$ real numbers $\mathbf{w}= [\textbf{w}_{1}, ..., \textbf{w}_{n}]$, a target function $f$ is a mapping from $\mathbf{X}$ to $\mathbf{y}$, i.e., $f(\mathbf{X}, \mathbf{w}): \mathbf{X} \times \mathbf{w} \rightarrow \mathbf{y}$. When the label {\bf y} takes on only a small number of {\it discrete} values {\it (e.g., two values: Rain (1) or No Rain (-1))}, the target function is for a {\it classification problem}. When the label we are trying to predict is continuous {\it (such as the specific inches of Rain)}, the target function is for a {\it regression} problem. 


\begin{exmp}
Consider \autoref{fig:1}, which uses a popular ML algorithm Support Vector Machine (SVM). The goal is to learn a linear boundary (margin) that separates the examples based on their Rain outcomes. The target function maps all examples in the input matrix to one of the two possible $\textbf{y}$ values [Rain, No Rain]. The classification {\bf target function}, $f(\mathbf{X}, \mathbf{w})$, is $\textbf{w}^T\textbf{X}$. 
\end{exmp}

\paragraph{{\bf Loss function}} $L(f(\textbf{X}, \textbf{w}), \textbf{y})$ is a measure of an algorithm's performance over all training examples. It characterizes how well an algorithm's {\it predictions} $f(\textbf{X}, \textbf{w})$ match the actual labels $\textbf{y}$, i.e., how well a model $\textbf{w}$ works. The exact form of the loss function depends on the choice of ML algorithm and target function.

\begin{exmp}
     For the SVM in \autoref{fig:1}, the \textbf{loss function} is defined as $L(f(\mathbf{X}, \mathbf{w}), \mathbf{y}) = \frac{1}{2}\|\mathbf{w}\|^2_2 + C\sum_{i=1}^{n}\max\{0, 1-y_i\mathbf{w}^T\mathbf{x}_i\}$. 

     Here, $\mathbf{w}^T\mathbf{x}_i$ represents the model's prediction for an example ${x}_i$, derived from the {\bf target function}, while $y_i$ denotes the actual label. When both predictions and labels share the same sign, the loss is low, indicating better algorithm performance. The notation $|| \cdot ||^2_2$ represents the squared Euclidean norm, and $C \in (0, +\infty)$ is a tunable parameter.
\end{exmp}



\paragraph{{\bf Model Training}} Taking an input matrix $\textbf{X}$ and a label vector $\textbf{y}$, a training algorithm \underline{$\mathcal{A}$ aims to return an optimal model $\textbf{w}^*$ that} \underline{minimizes the loss function}, i.e., $
\textbf{w}^* = \mathop{\arg \min}\limits_{\textbf{w}\in \mathcal{W}} L(f(\textbf{X}, \textbf{w}), \textbf{y})$For many non-convex problems where no algorithm guarantees a global minimum of loss function, such as Deep Neural Network (DNN), a good training algorithm returns a decent local minimum instead. 


\begin{exmp}
     For the SVM algorithm ($\mathcal{A}$) in \autoref{fig:1}, \textbf{optimal model} $\textbf{w}^*$ is the largest boundary to correctly separate the Rain and No Rain examples and therefore provides predictions equal to the actual labels i.e gives the minimum value for the loss function $L(f(\textbf{X}, \textbf{w}), \textbf{y})$.
\end{exmp}

\subsection{Missing Values and Repairs}
\noindent
\paragraph{{\bf Missing values}} Any $x_{ij}$ is a missing value (MV) if it is unknown (marked by \textit{null}).We denote the set of examples with missing values as $MV(x) = \{\textbf{x}_i | \exists x_{ij},  x_{ij} = \textit{null} \}$ and set of features with missing values as $MV(z) = \{\textbf{z}_j | \exists x_{ij},  x_{ij} = \textit{null} \}$.

\begin{exmp}
In \autoref{tab:missing_value}, the New York example's Humidity feature is missing value. Temperature is a missing-value-free (complete) feature, and Seattle is a complete example.
\end{exmp}

\paragraph{{\bf Complete values}} If a feature value is not \textit{null}, then it is complete. An example is complete if all its features are complete.



\paragraph{{\bf Repair}}A repair is a missing-value-free (complete) version of the raw data where all \textit{nulls} are replaced with values in $\mathbb{R}$. More formally: 
\begin{definition}(Valid Repair)
\label{definition_repair}
  For an input matrix $\textbf{X}$ having missing values. $\textbf{X}^{r}$ is a valid repair to $\textbf{X}$ if 1) $dimension(\textbf{X}^{r}) = dimension(\textbf{X})$, 2) $\forall x^r_{ij} \in \textbf{X}^r, x^r_{ij} \neq \textit{null}$, and 3) $\forall x_{ij}\neq\textit{null}$,  $x^{r}_{ij} = x_{ij}$.
\end{definition}

Further, since \textit{nulls} may be replaced with any value from $\mathbb{R}$ an infinite number of repairs may exist. Therefore, we denote the {\bf set of all possible repairs as  $\textbf{X}^{R}$}.

\begin{exmp}
In Table \ref{tab:missing_value}, the humidity feature for the New York \textbf{example} is a \textbf{missing value}. From Definition \autoref{definition_repair}, replacing the missing data with a value (e.g., $90 \in \mathbb{R}$) yields a valid repair (\textbf{X}$^r$). However, deleting the humidity feature, which eliminates the missing value, is not a valid repair since it changes dimension(X).

\end{exmp}


==> section8_algorithm_for_arccos_kernel_SVM_v1.tex <==
\section{Certain Models for DNN}\label{sec:DNN}
DNNs are popular ML models for a wide variety of tasks such as natural language processing and image classification.

Training a DNN involves solving very complex non-convex functions to learn nonlinear mappings for the input training examples~\cite{cho2011analysis}. This architecture makes it challenging to analyze the transformations the input examples (both complete and incomplete) go through.

As we have shown in Sections 5 and 6, analyzing SVM kernel families is achievable, as we can clearly see how the inputs are mapped. We know the functional form of the non-linear mapping.

Fortunately, some SVM kernel families have shown to approximate DNN computations~\cite{cho2011analysis}. For instance, the {\bf arc-cosine} kernel has been used to approximate different DNNs~\cite{cho2009kernel}. 

Therefore to approximate the {\bf conditions for having certain models for DNN} we formulate certain model conditions for SVM with arc-cos kernel. 
% DNNs represent state-of-the-art ML techniques across a wide spectrum of applications such as image classification, and the development of conversational ChatBots. They achieve such performance by processing input data through numerous layers (\textbf{`deep'}) of nonlinear transformations.

% DNNs require complex training involving challenging nonlinear optimizations and heuristics~\cite{cho2011analysis}. In contrast, kernel SVMs can learn nonlinear models (Section \ref{sec:kernel-SVM}) with much simpler training through {\it quadratic programming}.

% Some SVM kernel families offer a way to approximate DNN computations with {\bf `shallower structures'} ~\cite{cho2011analysis}. For instance, the {\bf arc-cosine} kernel has been used to approximate DNNs with different activation functions~\cite{cho2009kernel}. 

% Therefore to approximate the {\bf conditions for having certain models for DNN} we formulate certain model conditions for SVM with arc-cos kernel.

The arc-cosine ({\it arc-cos}) kernel function is defined as $k_{\text{arccos}}(\mathbf{x}_i, \mathbf{x}_j) = \pi - \cos^{-1}\left(\frac{\mathbf{x}_i \cdot \mathbf{x}_j}{|\mathbf{x}_i| \cdot |\mathbf{x}_j|}\right)$.

% In this section, our goal is to learn an efficient algorithm to check the existence and learn certain models for SVM with arc-cos kernel, so as to mimic the {\bf certain models for DNN}.

Similar to the RBF kernel, solving the minimization problem in Inequality \ref{eq:9} for the arc-cosine kernel is challenging (Subsection \ref{sec:Krbf}). To address this, we seek lower bounds, denoted as $lwb_i$. For all $\textbf{x}_i^r\in \textbf{x}_i^R$, we aim to satisfy: 
$$lwb_i \leq y_i\sum_{\textbf{x}_j \notin MV(\mathbf{x})} a_{j}^{\ddagger} y_j \\k_{arccos}(\textbf{x}_i^r, \textbf{x}_j)$$

However, obtaining $lwbi$ with theoretical guarantees is challenging. Because more than 1 cant guarrente all saddle points are global minimum, another non-convex problem.

Therefore, we focus on scenarios with a {\it single missing value per example}. So that the {\it stationary point} (where the gradient equals zero) of the kernel function is the global minimum. We leave the scenarios with multiple missing values per example as a future work.

Since Lemma 7.2 also applies to arc-cosine kernel, in order to efficiently find $lwb_i$ for all incomplete examples $\textbf{x}_i$, we need to compute$\mathop{\min}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}k_{arccos}(\textbf{x}_i^r, \textbf{x}_j)$ and $\mathop{\max}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}k_{arccos}(\textbf{x}_i^r, \textbf{x}_j)$without any repairs. We formalize this idea in the following theorem.

\begin{theorem}\label{theorem:DNN}
For arc-cosine kernel, the maximum and the minimum kernel function values between an incomplete example ($\textbf{x}_i^r$) and a complete example($\textbf{x}_j$) are as follows:
\begin{align*}
 \mathop{\max}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}k_{arccos}(\textbf{x}_i^r, \textbf{x}_j) = \pi - MAX[cos^{-1}(\frac{a}{c}), cos^{-1}(-\frac{a}{c})]
\end{align*}
\begin{align*}
 \mathop{\min}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}k_{arccos}(\textbf{x}_i^r, \textbf{x}_j) = \pi - cos^{-1}(\frac{a^2\cdot d + b^2}{c\cdot \sqrt{a^2\cdot d^2 + b^2 \cdot d}})
\end{align*}
Suppose $x_{iz} = \textit{null}$. To simplify notations, we define $a = x_{jz}$, $b = \sum_{x_{ip} \neq \textit{null}} x_{ip} \cdot x_{jp}$, $c = ||\textbf{x}_j||$, and $d = \sum_{x_{ip} \neq \textit{null}} x_{ip}^2$.
\end{theorem}

\begin{proof}
Consider the arc-cosine term of the kernel function, $cos^{-1}(\frac{\textbf{x}^r_i \cdot \textbf{x}_j}{||\textbf{x}^r_i||\cdot||\textbf{x}_j||})$. Based on the property of the arc-cosine function: 
\[
arg\mathop{\max}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}cos^{-1}(\frac{\textbf{x}^r_i \cdot \textbf{x}_j}{||\textbf{x}^r_i||\cdot||\textbf{x}_j||}) =arg\mathop{\min}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}\frac{\textbf{x}^r_i \cdot \textbf{x}_j}{||\textbf{x}^r_i||\cdot||\textbf{x}_j||}
\]
And vice versa. So we define a function
\[
f(x^r_{iz}) =\frac{a\cdot x^r_{iz} + b}{c \cdot \sqrt{(x^r_{iz})^2 + d}}
\]
Taking the derivative of the $f(x^r_{iz})$ with respect to the repair $x^r_{iz}$:
\[
f(x^r_{iz})' = \frac{a}{c \cdot \sqrt{(x^r_{iz})^2 + d}} - \frac{a\cdot (x^r_{iz})^2 + b\cdot x^r_{iz}}{c \cdot\sqrt{[(x^r_{iz})^2 + d]^3}}
\]
Through some simple derivation, one can find $f'(x^r_{iz}) \geq 0$ when $x^r_{iz} \leq \frac{a\cdot d}{b}$, and $f'(x^r_{iz}) \leq 0$ when $x^r_{iz} \geq \frac{a\cdot d}{b}$. This means that $x^r_{iz} = \frac{a\cdot d}{b}$ is the only stationary point that gives us the global minimum of $f(x^r_{iz})$. And the maximum is reached at either $x^r_{iz} = -\infty$ or $x^r_{iz} = +\infty$. Finally, bringing these maximum and minimum for $f(x^r_{iz})$ to the kernel function, we can find $\mathop{\min}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}k_{arccos}(\textbf{x}_i^r, \textbf{x}_j)$ and $\mathop{\max}\limits_{\textbf{x}_i^r\in \textbf{x}_i^R}k_{arccos}(\textbf{x}_i^r, \textbf{x}_j)$ as outlined in Theorem 8.1.
\end{proof}

Theorem shows ....this provides us an insight .... on future directions. 
% \subsection{Checking and Learning Certain Models} Given the similarity of conditions for having certain models between RBF kernel and arc-cosine kernel we can easily modify Algorithm 4 to get the algorithm for arc-cosine SVM.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%If removing the pseudo-code

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% If $y_i \cdot a_{j}^{\ddagger} \cdot y_j > 0 $ then $lwb_i \gets y_i \cdot a_{j}^{\ddagger} \cdot y_j \cdot [\pi - cos^{-1}(\frac{a^2\cdot d + b^2}{c\cdot \sqrt{a^2\cdot d^2 + b^2 \cdot d}})]$ Else $ lwb_i \gets y_i \cdot a_{j}^{\ddagger} \cdot y_j \cdot \{\pi - MAX[cos^{-1}(\frac{a}{c}), cos^{-1}(-\frac{a}{c})]\}$  $lwb_i \gets y_i \cdot a_{j}^{\ddagger} \cdot y_j \cdot [\pi - cos^{-1}(\frac{a^2\cdot d + b^2}{c\cdot \sqrt{a^2\cdot d^2 + b^2 \cdot d}})]$ and $ lwb_i \gets y_i \cdot a_{j}^{\ddagger} \cdot y_j \cdot \{\pi - MAX[cos^{-1}(\frac{a}{c}), cos^{-1}(-\frac{a}{c})]\}$ 

% Based on Theorem \ref{theorem:DNN}, we present Algorithm \ref{alg:kARCCOS} for checking and learning certain models for DNN. This algorithm is different than Algorithm \ref{alg:kRBF}, only in terms of how the lower bound $lwbi$ is computed. The time complexity of this algorithm is also $\mathcal{O}(T_{train})$.

%to check the existence of a certain model efficiently with Algorithm \autoref{alg:kARCCOS}. If a certain model is determined to exist, $\textbf{a}^{\ddagger}$ is exactly the certain model. 
% Theorem 5.1 says that a certain model exists for a linear regression if and only if the residue vector $\textbf{r}$ is orthogonal to features with missing values. If a certain model exists, the missing features can be safely ignored without compromising the minimization of training loss since they do not contribute to a smaller training loss than $\textbf{r}$.

% Theorem 8.1 essentially says, 


% \begin{algorithm}
% \caption{Checking and learning certain models for $k_{arccos}$ SVM}\label{alg:kARCCOS}
% \begin{algorithmic}

% \State $MV(\mathbf{x}) \gets \text{incomplete examples}$
% \State $ \textbf{a}^{\ddagger} \gets 
% \text{the model trained with complete training examples}$

% \For {$\textbf{x}_i \in MV(\mathbf{x})$}
%     \State $a \gets x_{jz}$, $b \gets \sum_{x_{ip} \neq \textit{null}} x_{ip} \cdot x_{jp}$
%     \State $c \gets ||\textbf{x}_j||$, $d \gets \sum_{x_{ip} \neq \textit{null}} x_{ip}^2$
%     \For {$\textbf{x}_j \notin MV(\mathbf{x})$}
%         \If{$y_i \cdot a_{j}^{\ddagger} \cdot y_j > 0 $} 
%             \State $lwb_i \gets y_i \cdot a_{j}^{\ddagger} \cdot y_j \cdot [\pi - cos^{-1}(\frac{a^2\cdot d + b^2}{c\cdot \sqrt{a^2\cdot d^2 + b^2 \cdot d}})]$
%         \Else
%             \State $ lwb_i \gets y_i \cdot a_{j}^{\ddagger} \cdot y_j \cdot \{\pi - MAX[cos^{-1}(\frac{a}{c}), cos^{-1}(-\frac{a}{c})]\}$        
%         \EndIf
%     \EndFor   
% \EndFor
% \If{$MIN(lwb_1, lwb_2, ...) > 1$}
%     \State \Return \text{"A certain model $\textbf{a}^{\ddagger}$ exists"}
% \EndIf
% \end{algorithmic}
% \end{algorithm}
    

==> section9_empirical_approach.tex <==
\section{Empirical Approach measuring the uncertainty caused by missing data}
As an analytical approach, checking certain models avoids materializing all repairs when measuring uncertainty in ML models caused by missing data. However, there are two limitations: 1) For many ML models, it is hard to find an efficient algorithm for checking certain models, and 2) Certain models do not often exist. To note, "no certain models exist" does not necessarily mean "a high uncertainty in ML model performance". Therefore, a general and empirical approach is needed to address the limitations and complement the analytical approach. 
\begin{figure*}\label{fig:2}
  \includegraphics[width=\textwidth]{images/pipeline.png}
   \caption{Proposed Empirical Approach to Measure Uncertainty in ML Model Performance from Missing Data }
\end{figure*}

\subsection{Pipeline for Uncertainty Measurement}
Figure 2 demonstrates a pipeline to measure uncertainty in model performance caused by missing data. Starting with raw data with missing values, we first randomly split data into three sets (training, validation, and testing). In the baseline algorithm in Section \ref{sec4}, all possible models are trained from a large number of repairs. This algorithm is correct but not feasible in implementation as it involves training a large number of possible models. Therefore, we sample a sufficient number ($t$) of repairs to the training set and then use each repair to train a model individually. As a result, we get $t$ models from $t$ repair samples. To evaluate the uncertainty in model performance, we discover the difference between the $t$ models in terms of validation accuracy. However, the validation set also contains missing values that bring in uncertainty. Therefore, we also sample a sufficient number ($u$) of repairs to the validation set. Then, we compute validation accuracy between $t$ models and $u$ validation repairs pairwise: for each one of the $t$ models, compute validation accuracy with respect to each one of the $u$ validation repairs. At this point, there should be $t\cdot u$ validation accuracies. The variance within the $t\cdot u$ validation accuracies reflects the uncertainty in model validation caused by missing data. If the variance is large, we may consider data cleaning. If the variance is small, we should expect similar model validation results from any two possible models. 

Upon model validation, an optimal model is selected for the final testing. Many works assume a clean testing set in their frameworks although this is not often the case in practice: the testing set usually also contains missing values. Hence, similar to the validation set, we can also sample a sufficient number ($v$) of repairs to the testing set, and compute the testing accuracy of the optimal model with respect to all $v$ test repairs individually. By evaluating the difference in the $v$ testing accuracies, we measure the uncertainty of the optimal model in terms of testing performance.

\subsection{Optimization of the Pipeline}
This empirical approach is general to most ML models. However, one may find the pipeline not efficient since it involves sampling a large amount of repairs and then training a large number of models. To address the issue, we propose some solutions to optimize the pipeline. 
\subsubsection{Optimization in Sampling}
The main goals in the sampling stage are: 1) as few repairs as possible for a light computational overhead, and 2) the repair samples reflect the real distribution for each missing value. For example, the humidity in New York is missing in Table \ref{tab:missing_value}, and suppose the humidity in a city follows the normal distribution with mean of $u$ and variance of $\delta$. We would like repair samples to also follow this normal distribution. To achieve goal 1), we use Markov Chain Monte Carlo methods (MCMC), specifically Gibbs Sampling \cite{gibbs_sampling} in order to efficiently sample from a world of possible repairs. (Details are to be merged from Amandeep's project report upon a notation fix for consistency). To achieve goal 2), for each missing feature (e.g., the temperature in Table \ref{tab:missing_value}), we simulate the distribution of the feature value based on non-missing values in the feature. Then, at Gibbs sampling, we incorporate the simulated distributions in repair generation. 

\subsubsection{Optimization in Training}
The most time-consuming process in the pipeline is training a large number of models individually. The training cost linearly grows as the number of repairs grows. In the paper, we propose two techniques to save costs by sharing computation between training models with different repairs. Firstly, the warm starting strategy is employed to offer a decent initialization while training $m$ models in the pipeline. Basically, in warm starting, we save the model trained from the last repair and set it as the initialization when training a new model with the next repair. The strategy assumes that minor changes in training data bring minor changes in model optimality, and has been demonstrated with excellent cost savings in many work\cite{ash2020warm, he2014practical}. Warm starting is expected to work very well with the repair samples generated by Gibbs sampling because the difference between one repair to another is extremely minor: only one value is changed between two adjacent repairs. 

In addition, we employ other incremental learning techniques (TO BE UPDATED)
\subsubsection{Optimization in Inference}
(Note: This is from the idea we talked about at the last meeting---how to save costs for validation and in what condition do similar model parameters lead to similar model prediction accuracies)\\
Although the costs for inference from model validation are much smaller than model training, there is still room to save. For example, in SVM, predictions are made based on the decision function $f(\textbf{X}, \textbf{w}) = sign(\textbf{X}\textbf{w})$ which returns binary label outputs ($\pm 1$) from the validation data. Suppose there are $u$ validation repairs, the baseline algorithm for performing validation is: individually computing the validation accuracy for $u$ repairs by running the decision function for $u$ times. The time complexity for the baseline algorithm is $\mathcal{O}(u\cdot m\cdot d)$, suppose there are $m$ examples in the validation set, and each example has $d$ features. Since two adjacent validation set repairs are different on only one value based on Gibbs sampling, efforts can be saved by sharing computation between predicting one validation repair to another. Specifically, we run the decision function for the first repair $\textbf{X}^{r1}$ which returns the validation result $\textbf{y}^{r1} = sign(\textbf{X}^{r1}\textbf{w})$. Then, we get the second repair from Gibbs sampling, $\textbf{X}^{r2}$, where its only difference with $\textbf{X}^{r1}$ is $x^{r1}_{ij} \neq x^{r2}_{ij}$. Instead of running the decision function again for $\textbf{X}^{r2}$, we can directly get the validation result $\textbf{y}^{r2}$ by a computationally efficient update from $\textbf{y}^{r1}$. This is because $\textbf{y}^{r2}$ and $\textbf{y}^{r2}$ have at most one different label on $y^{r1}_i \neq y^{r2}_i$ because $\textbf{w}^T\textbf{x}^{r1}_i \neq \textbf{w}^T\textbf{x}^{r2}_i$:
\begin{align*}
     \textbf{y}^{r2} & = [y^{r2}_1, ..., y^{r2}_i, ..., y^{r2}_m]^T \\ 
     & = [y^{r1}_1, ..., sign\{\textbf{w}^T\textbf{x}^{r1}_i + w_i(x^{r2}_{ij} - x^{r1}_{ij})\}, ..., y^{r1}_m]^T   
\end{align*}


where $\textbf{w}^T\textbf{x}^{r2}_i$ is computed by $\textbf{w}^T\textbf{x}^{r1}_i + w_i(x^{r2}_{ij} - x^{r1}_{ij})$, and $\textbf{w}^T\textbf{x}^{r1}_i$ is saved from the last predicting with $\textbf{X}^{r1}$. As a result, we only need to run the prediction function for the first repair and implement minor updates for the following repairs. This optimization leads to a time complexity of $\mathcal{O}(u + m\cdot d)$, which is much smaller than $\mathcal{O}(u\cdot m\cdot d)$ from the baseline algorithm if the number of validation repairs is large. 

Similar ideas about the optimization also apply to other linear models such as linear regression, and can potentially be extended to neural networks (WORKING ON IT)

==> section9_possible_models.tex <==
\section{Possible Models}
Certain Models while immensely powerful rarely exist in the real world datasets, the conditions for certain models to exist are quite stringent. This makes them quite difficult to find and utilize in the real world datasets. 
However, they can serve as foundational building blocks for defining a broader range of models with less restrictive conditions for their existence. In this section, our goal is to formally define these possible models and develop an algorithm capable of efficiently computing and identifying sets of such models.

\subsection{Defining Possible Models}
Expanding on the concept of repairs, we can define:
\begin{definition}
    A set of possible repairs $\mathcal{I}_X$ is a collection of all repairs $\mathcal{X}^r$ that satisfy the conditions of being a valid repair.
\end{definition}

Instead of getting a deterministic model $\textbf{w}$ through data cleaning, we can leave missing data as-is and incorporate the uncertainty in models by treating all model parameters $w_1, ..., w_n$ as random variables. To be specific, each model parameter $w_i$ is represented by a probability density function $p(w_i)$. The idea is illustrated by possible models, with the following definition. Denote $w_i^r$ by the $i^{th}$ model parameter learned with repair $\mathcal{X}^r$, 
i.e., $\mathcal{A}(\mathcal{X}^r) = \textbf{w}^r = [w_1^r, ..., w_n^r]$

\begin{theorem}\label{thm:pm}
    A model $\textbf{w} = [p(w_1), ..., p(w_n)]$ is be determined as a possible model if $\forall i \in [1, ..., n]$ these two conditions are met: 1) $p(w_i)$ is a probability density function; 2) $Pr(a \leq w_i^r \leq b, \forall \mathcal{X}^r \in \mathcal{I}_X) = \int_{a}^{b} p(w_i) \,dw_i $
\end{theorem}


In a possible model, $p(w_i)$ represents the probability density for the $i^{th}$ model parameter. This distribution characterizes the amount of uncertainty projected from the missing data into this particular model parameter. For example, if $p(w_i)$ has a very small variance, learning from any repair is likely to yield similar $w_i$ values. If all model parameters have low-variance distributions, data cleaning may not be necessary since the uncertainty in the model is sufficiently small. Essentially, the uncertainty in $\mathcal{I}_X$ due to missing data is translated into the possible models via a training algorithm $\mathcal{A}$.

\subsection{Computing Possible Models}
However, calculating the probability density functions $p(w_i)$ is challenging because the size of $\mathcal{I}_X$ is often infinite. Therefore, it is intuitive to approximate the distributions through repair sampling: 1) sample a sufficient number of repairs $\mathcal{X}^r$, 2) train the model $\textbf{w}^r$ from each sampled repair, and 3) fit the probability distributions $p(w_i)$ using the obtained $\textbf{w}^r$ values.

Ideally, we aim to sample a small number of repairs and ensure that the models trained from these repairs are representative. This approach allows us to obtain well-fitted probability distributions with minimal sampling and training costs. We utilize Markov Chain Monte Carlo methods (MCMC), specifically Gibbs Sampling \cite{gibbs_sampling} in order to efficiently sample from a world of possible repairs. 

Algorithm \ref{alg:possible_svm} outlines the step-by-step process used to discover possible models for a linear-SVM problem. In this algorithm, we employ the Kullback-Leibler Divergence (KL divergence) method to compare the probability density functions of the repairs. This comparison serves as a stopping condition for the algorithm, which is based on a user-defined hyperparameter $\delta$.

The goal of the algorithm is to iteratively sample and train models from repairs, and then evaluate the similarity between their probability density functions using the KL divergence. As long as the KL divergence between consecutive iterations remains above the specified threshold $\delta$, the algorithm continues. Once the KL divergence falls below $\delta$, indicating that the probability density functions have converged sufficiently, the algorithm terminates.

By using the KL divergence as a stopping condition, we can control the level of similarity required between the probability density functions of the repairs to ensure convergence. This approach provides a clear criterion for ending the algorithm and obtaining the set of possible models for the linear-SVM problem.

\begin{algorithm}
\caption{Possible models for SVM}\label{alg:possible_svm}
\begin{algorithmic}
\State $D \gets \text{the training dataset}$
\State $MV \gets \text{set of indices for missing values}$
\State $n \gets \text{the number of samples}$
\State $b \gets \text{the batch size}$
\State $\delta \gets \text{the KL-divergence threshold}$
\State $D_0 \gets \text{Dataset with } MV \text{ imputed with random constant } c$
\State $\textbf{w}_0 \gets \text{Train SVM on } D_0$
\State $res \gets False$

\For {$epoch \in \{0, 1, ..., n\}$}
    \State $D_b \gets \text{Random batch from } D_0$
    \State $D_{b_s} \gets \text{repair sampled with Gibbs Sampling}$
    \State $\textbf{w}_{epoch} \gets \text{Update SVM on } D_{b_s}$
    \State $p_{\textbf{w}} \gets pdf(\textbf{w})$
    \State $p_{\textbf{w}_{epoch}} \gets pdf(\textbf{w}_{epoch})$
    
    \If {$\text{KL}(p_{\textbf{w}_0}, p_{\textbf{w}_{epoch}}) \leq \delta$}
        \State $res \gets True$
        \State \textbf{break}
    \EndIf
    \State $\textbf{w} \gets \textbf{w} \cup \textbf{w}_{epoch}$
\EndFor

\State \Return $p(\textbf{w})$
\end{algorithmic}
\end{algorithm}

\paragraph{}
The algorithm computes and returns $p(\textbf{w})$ as a $pdf$ of a set of possible models which can approximately minimize the loss function without cleaning. We demonstrate the efficiency and robustness of the algorithm in Section \ref{sec6}.
